Learning with Pseudo-Ensembles

We formalize the notion of a pseudo-ensemble, a (possibly infinite) collection of child models spawned from a parent model by perturbing it according to some noise process. E.g., dropout (Hinton et. al, 2012) in a deep neural network trains a pseudo-ensemble of child subnetworks generated by randomly masking nodes in the parent network. We present a novel regularizer based on making the behavior of a pseudo-ensemble robust with respect to the noise process generating it. In the fully-supervised setting, our regularizer matches the performance of dropout. But, unlike dropout, our regularizer naturally extends to the semi-supervised setting, where it produces state-of-the-art results. We provide a case study in which we transform the Recursive Neural Tensor Network of (Socher et. al, 2013) into a pseudo-ensemble, which significantly improves its performance on a real-world sentiment analysis benchmark.

==> PE-math.tex <==

The authors of \cite{Wager2013} (abbr.~WWL) show that, given some assumptions\footnote{They assume a noise process $\xi$ such $\expect_{\xi} [ f(x; \xi) ] = f(x)$, i.e.~one which doesn't affect the expectation of $f(x)$.}, logistic regression under the influence of dropout is equivalent to the following regularized objective:
\begin{equation}
\sum_{i=1}^{n} \expect_{\xi} \left[ \ell(f_{\theta}(x_i; \xi), y_i) \right] = \sum_{i=1}^{n} \ell(f_{\theta}(x_i), y_i)) + R(f_{\theta}), 
\label{wwl_obj}
\end{equation}
in which $f_{\theta}(x_i) = \theta x_i$, $\ell(f_{\theta}(x_i), y_i)$ is the logistic regression loss for prediction $f_{\theta}(x_i)$ given true class $y_i$, $f_{\theta}(x_i; \xi)$ indicates computing $f_{\theta}$ subject to perturbation by the \emph{noise process} $\xi$, and the regularization term $R(f_{\theta})$ is given by:
\begin{equation}
R(f_{\theta}) \equiv \sum_{i=1}^{n} \expect_{\xi} \left[ A(f_{\theta}(x_i; \xi)) - A(f_{\theta}(x_i)) \right],
\label{wwl_reg}
\end{equation}
where $A(\cdot)$ indicates the log partition function for logistic regression.


When using the KL-divergence penalty, PEV-regularized logistic regression minimizes:
\begin{equation}
\sum_{i=1}^{n} \ell(f_{\theta}(x_i), y_i) + \expect_{\xi} \left[ \DD_{KL} \left(\softmax(f_{\theta}(x_i)) \, || \, \softmax(f_{\theta}(x_i; \xi)) \right) \right],
\label{pev_obj}
\end{equation}
in which $\softmax(\cdot)$ indicates the standard softmax function, and $\DD_{KL}(p \, || \, \tilde{p})$ indicates the KL-divergence between ``true'' distribution $p$ and ``approximate'' distribution $\tilde{p}$, i.e.:
\begin{equation}
\DD_{KL}(p \, || \, \tilde{p}) = \sum_{c \in C} p(c) \log \frac{p(c)}{\tilde{p}(c)}
\label{kl_div}
\end{equation}
for distributions $p/\tilde{p}$ over the set of possible classes in $C$. We now define distribution $p_{\theta}(x)$ as $\softmax (f_{\theta}(x))$, which is given by:
\begin{equation}
p^{c}_{\theta}(x) = \frac{\exp f^{c}_{\theta}(x)}{\sum_{c^{\prime} \in C} \exp f^{c^{\prime}}_{\theta}(x)} ,
\label{quiet_probs}
\end{equation}
where we assume $x \in \Real^{n \times 1}$, $\theta \in \Real^{|C| \times n}$, $f_{\theta}(x) \in \Real^{|C| \times 1}$, $p_{\theta}(x) \in \Real^{|C| \times 1}$, and we use superscripts to indicate particular elements in a vector. Similarly, we define $p_{\theta}(x; \xi)$ such that:
\begin{equation}
p^{c}_{\theta}(x; \xi) = \frac{\exp f^{c}_{\theta}(x; \xi)}{\sum_{c^{\prime} \in C} \exp f^{c^{\prime}}_{\theta}(x; \xi)}.
\label{noisy_probs}
\end{equation}

Given the definitions provided above, we now show that PEV regularization with a KL-divergence penalty on the outputs of the pseudo-ensemble reproduces the effect of dropout when $\expect_{\xi} [f_{\theta}(x; \xi)] = f_{\theta}(x)$. We simply rewrite the PEV part of Equation \ref{pev_obj} using the expanded forms in Equations \ref{kl_div}--\ref{noisy_probs}:
\begin{eqnarray}
&\;& \expect_{\xi} \left[ D_{KL} \left(p_{\theta}(x) \, || \, p_{\theta}(x; \xi) \right) \right] \\
&=& \expect_{\xi} \left[  \sum_{c \in C} p^{c}_{\theta}(x) \log \frac{p^{c}_{\theta}(x)}{p^{c}_{\theta}(x; \xi)} \right] \\
&=& \sum_{c \in C} \expect_{\xi} \left[ p^{c}_{\theta}(x) \log \frac{ \exp f^{c}_{\theta}(x) \sum_{c^{\prime} \in C} \exp f^{c^{\prime}}_{\theta}(x; \xi) }{ \exp f^{c}_{\theta}(x; \xi) \sum_{c^{\prime} \in C} \exp f^{c^{\prime}}_{\theta}(x) } \right] \\
&=& \sum_{c \in C} \expect_{\xi} \left[ p^{c}_{\theta}(x) \left( (f^c_{\theta}(x) - f^c_{\theta}(x; \xi)) + (\log \sum_{c^{\prime} \in C} \exp f^{c^{\prime}}_{\theta}(x; \xi) - \log \sum_{c^{\prime} \in C} \exp f^{c^{\prime}}_{\theta}(x) ) ) \right) \right] \\
&=& \sum_{c \in C} \expect_{\xi} \left[ p^{c}_{\theta}(x) (f^c_{\theta}(x) - f^c_{\theta}(x; \xi)) + p^{c}_{\theta}(x)  (A(f_{\theta}(x; \xi)) - A(f_{\theta}(x))) \right] \\
&=& \expect_{\xi} \left[ \sum_{c \in C} p^{c}_{\theta}(x)  (A(f_{\theta}(x; \xi)) - A(f_{\theta}(x))) \right] \\
&=& \expect_{\xi} \left[ A(f_{\theta}(x; \xi)) - A(f_{\theta}(x)) \right]
\label{pev_reg_expanded}
\end{eqnarray}
which brings us to the regularizer described by WWL, and as written in Equation \ref{wwl_reg}. We now briefly explain each step in this transformation:
\begin{itemize}
\item $7 \rightarrow 8$: By definition of KL-divergence.
\item $8 \rightarrow 9$: By definition of the $p_{\theta}$s and by swapping an expectation and a sum.
\item $9 \rightarrow 10$: By well-known properties of $\log$ and $\exp$.
\item $10 \rightarrow 11$: By distributivity and by definition of logistic regression's log-partition function.
\item $11 \rightarrow 12$: By assumption that $\expect_{\xi} [f_{\theta}(x; \xi)] = f_{\theta}(x)$ and by expectation/sum swapping.
\item $12 \rightarrow 13$: By independence of $A(f_{\theta}(x; \xi)) - A(f_{\theta}(x))$ from $c$ and $\sum_{c \in C} p^{c}_{\theta}(x) = 1$.
\end{itemize}

So, some basic algebra shows that PEV regularization via KL-divergence of the pseudo-ensemble members is equivalent to dropout whenever the noise process $\xi$ generates the pseudo-ensemble such that $\expect_{\xi} [f_{\theta}(x; \xi)] = f_{\theta}(x)$, and assuming a logistic regression ``primary'' objective.


